CodemixedNLP: An Extensible and Open NLP Toolkit for Code-Mixing

The NLP community has witnessed steep progress in a variety of tasks across the realms of monolingual and multilingual language processing recently. These successes, in conjunction with the proliferating mixed language interactions on social media have boosted interest in modeling code-mixed texts. In this work, we present CodemixedNLP, an open-source library with the goals of bringing together the advances in code-mixed NLP and opening it up to a wider machine learning community. The library consists of tools to develop and benchmark versatile model architectures that are tailored for mixed texts, methods to expand training sets, techniques to quantify mixing styles, and fine-tuned state-of-the-art models for 7 tasks in Hinglish. We believe this work has a potential to foster a distributed yet collaborative and sustainable ecosystem in an otherwise dispersed space of code-mixing research. The toolkit is designed to be simple, easily extensible, and resourceful to both researchers as well as practitioners.

==> images/toolkit.tex <==
\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{images/toolkit_ui.png}
\caption{\label{fig:toolkit_ui} 
Our toolkit's web interface. The top image corresponds to the Homepage where the user can select a model of their choice. The bottom image shows the model specific UI. 
}
\bigbreak
\includegraphics[width=0.5\textwidth]{images/toolkit_cmd.png}
\caption{\label{fig:toolkit_cmd} 
Our toolkit's command line interface. We provide several functionality compatible with the popular Huggingface and Fairseq libraries.
}
\end{figure}

==> images/toolkit_ui.tex <==
\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{images/tool.png}
\caption{\label{fig:toolkit_ui} 
\small Our toolkit's web interface. The top image corresponds to the Homepage where the user can select a model of their choice. The bottom image shows the model specific UI. 
}
\end{figure}

==> sections/notes.tex <==
\section{Notes}
\label{sec:notes}

Why do we need this:
\begin{itemize}
    \item Lots of growing interest in NLP for Hinglish, due to its increasing presence in social media like Twitter, Youtube, Facebook, etc. Several new datasets and shared tasks created in recent years to advance studies for Hinglish. 
    \item With the successes of monolingual and multilingual transformer-based pretrained models like BERT, previous works obtained a preliminary understanding that multilingual pretrained models are capable of performing better for Hinglish. But their analysis has been largely limited to certain pretrained models. Thus, a need for comprehensive understanding as to which model performs better for Hinglish.
    \item In a parallel, several toolkits have emerged recently for supporting token-level language identification for Hinglish texts. But these toolkits do not use transformer based models, which are shown to perform better. Even if such exist, they are not easily adaptable into a downstream application.
    \item There is a dearth of toolkits for several other tasks in NLP, such as Hate speech detection, sentiment analysis, aggression identification, etc. Owing to their different creation strategies, the datasets for these tasks are spread out, and so are the model evaluations. 
    \item At this juncture, it is also important that different datasets be dealt in a common data format to facilitate comprehensive benchmarking.
    Hence a need for an \textit{umbrella} toolkit to facilitate easy benchmarking, better pretrained model evaluation and adaptations to downstream applications.
    \item Due to the peculiarity of mixing (and hence their differences with monolingual and multilingual NLP), it is important to understand if different representation techniques can improve Hinglish comprehension, and if yes to what extent.
    \item The contribution so this paper are four fold:
    \begin{itemize}
    \item A comprehensive benchmarking of different pretrained models for a variety of codemixed datasets, spanning semantic and syntactic tasks.
    \item Making the best performing models open for usage in industry/academia in a way that is easily extensible and adaptable to downstream NLP applications.
    \item Populating the toolkit with a variety of model architectures, consisting of both popularly utilized transformer architectures as well as some tailored for mixing scenarios.
    \item Making available different assets for data augmentation, transliterations, pretraining, 
    \end{itemize} 
    
\end{itemize}



 %Although we have  are good, we still lack a comprehensive understanding. For example, it is always better to input text in romanized or can these models comprehend native script equally better?, or are these models already aware of inconsistent spelling variations, etc. Amidst this, there are growing NLP tools for Indic and specifically Hinglish language, like transliterators, words normalizers, etc. This toolkit is motivated to advance NLP studies in Hinglish NLP by creating a unified platform to understand and benchmark pretrained models better, as well as make the best of these models available for public usage. This toolkit can also be used to develop new models, to validate performances across different datasets, to serve models with differet text forms eg. transliterated texts (by reusing existing tools), to understand the patterns of code-mixing in a given dataset, etc.

\begin{itemize}[noitemsep]
    \item Code formatting
        \begin{itemize}[noitemsep]
            \item \textit{model\_type} and \textit{model\_name} to be introduced
            \item {
                Create a base class and more classes. A model creator
                creates the right model, has the list of vocab to load,
                required set of optimizers, etc. See example below.
            }
            \begin{lstlisting}
                MODEL_DICT = {
                    "model_name": (
                        .models.model_class, 
                        (label_vocab, lid_vocab, etc.), 
                        (bert_optimizer, adam_optimizer)
                        )
                }
            \end{lstlisting}
            \item saving based on some necessary properties of the model, instead of all args
        \end{itemize}
    \item Add features to toolkit
        \begin{itemize}[noitemsep]
            \item decide on datasets and tasks
            \item Task adaptive pretraining for BERT based models
            \item Word-level LID is still a useful tool. Check if there are tools for it.
                    Example: deep learning based repos in github, LINCE github repo, 
                                microsoft LID tool
                    Issues w/ these: Some need training, some give sub-word level,
                                    some require external dependencies.
            \item Similar sentences feature. Use dataset creation strategy from 
                    XNLI and use BERT models to train using sentence-transformers 
                    (Idea from \citet{url1})
            \item Data augmentation- through transliterations, similar task datasets, noising by character level modifications
            \item releasing domain adapted models
            \item analysis tools- cs index, sub-sample some examples and evaluate, etc.
        \end{itemize}
    \item CodemixedNLP instead of HinglishNLP
        \begin{itemize}[noitemsep]
            \item Transliterators (Khyathi ma'am suggested repo for Indic languages). Look for Arabic, Spanish transliterators
        \end{itemize}
\end{itemize}


==> tables/pretrained_models.tex <==
\begin{table}[]
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
Task Type  & Task Name                                                                 \\ \hline
Semantic   & \makecell[l]{Sentiment Classification, Hate Speech\\Identification and Aggression Identification} \\ \hline
Syntactic  & NER, POS and Language Identification                                 \\ \hline
Generation  & Machine Translation (Hinglish$\rightarrow$English)                                 \\ \hline
% Generation & Machine Translation                                                      \\ \hline
\end{tabular}%
}
\caption{List of tasks in Hinglish for which fine-tuned models are readily available for usage in our toolkit}
\label{tab:pretrained_models}
\end{table}
